QGeo: A Python package for calculating geodesic control functions for quantum computing

We present a new Python package that uses the established notion of geometric quantum complexity to numerically compute the difficulty associated with preparing a given unitary transformation on a quantum computer. The numerical procedure we implement is presented and discussed. Analyzed quantum circuits include: the quantum fourier transform for up to four qubits, a random circuit with depth 100, and a circuit for analyzing the evolution of a fermionic chain with several lattice sites. This package can be found for download at https://github.com/JAGDiaz/quantum-geodesics

==> sections/section02p5.tex <==
\section{Geometrical Picture} \label{sec:geometrical_picture}

 
    The geometry of the qubit computational complexity problem takes place on the manifold and Lie group $SU\left(2^{n}\right)$ where $n$ is the number of qubits being utilized. Let $U$ be an element of $SU\left(2^{n}\right)$; in physical terms,  $U$ is a unitary operator which time evolves a wave function. We note that for a general qubit gate that any $U$ in $U\left(2^{n}\right)$ can be moved from $U\left(2^{n}\right)$ by a global phase into being an element of $SU\left(2^{n}\right)$. This is important because often target unitaries are given as elements in $U\left(2^{n}\right)$, but physically we only prepare elements in $SU(2^n)$ because global phases are not observable without introducing ancillary qubit registers.
    
    A tangent vector to a point $p$ on $SU\left(2^{n}\right)$  is an element of the Lie algebra $\mathfrak{su}\left(2^{n}\right)$. Let $H$ be a traceless $2^{n}\times2^{n}$ Hermitian matrix. Then, $iH$ is an element of $\mathfrak{su}\left(2^{n}\right)$; we call this $H$ the Hamiltonian because it generates the time evolution of $U$
    
    To draw an analogy to connecting the identity operator to a target unitary, we give a brief description of a geometric flow on a manifold. We will think of a time-dependent vector field $f$ on $SU\left(2^{n}\right)$ as a smooth map such that for all $t\in\mathbb{R}$, $p\in SU\left(2^{n}\right)$, $f\left(t,p\right)\in \mathfrak{su}\left(2^{n}\right)$. Let $I\subseteq\mathbb{R}$ be an interval containing $0$, then the flow of $f$ is a function $\phi:I\times SU\left(2^{n}\right)\rightarrow{}SU\left(2^{n}\right)$ satisfying equations \eqref{eq:Flow}.

    \begin{align}
        \label{eq:Flow}
        \phi\left(0,x_{0}\right)=x_{0}\\ \nonumber
        \left.\dot{\phi}\left(t,x_{0}\right)\right|_{t=t_{0}}=f\left(t_{0},\phi\left(t_{0},x_{0}\right)\right)\\ \nonumber
        \forall x_{0}\in\ SU\left(2^{n}\right),\ \ \ t_{0}\in I
    \end{align}


     with initial condition $U_{0}=\mathbb{1}$, $\mathbb{1}$ being the identity matrix of proper dimension, defines a flow on $SU\left(2^{n}\right)$ where $-\frac{i}{\hbar}H=f$ is the operator on $U\left(t\right)$. We give a comparison below to cement the analogy.

    \begin{align}
        \label{eq:Schrodinger as flow}
        U\left(0,\mathbb{1}\right) = \mathbb{1}\\ \nonumber
        \left.\dot{U}\left(t,\mathbb{1}\right)\right|_{t=t_{0}}=-\frac{i}{\hbar}H\left(t_{0},U\left(t_{0},\mathbb{1}\right)\right)\\ \nonumber
        \mathbb{1}\in\ SU\left(2^{n}\right),\ \ \ t_{0}\in I
    \end{align}
    
    To this end, we can think of flowing out from the identity to a target unitary as defining a curve which tells us how our qubits will evolve over time.
   
    \subsubsection{The Lifted Jacobi Equation and Minimizing Complexity}

    We define the lifted Jacobi field $J\left(t\right)\in T_{\gamma\left(t;0\right)}M$, the tangent space to a geodesic $H\left(t;0\right)$ of M=$\mathfrak{su}\left(2^{n}\right)$, by

    \begin{align}
        J\left(t\right)=\left.\frac{\partial}{\partial s}H\left(t;s\right)\right|_{s=0},
    \end{align}

    where we think of $s$ as the penalty parameters. The vector field, $J$ obeys an equation of the form:

    \begin{align}
        \label{eq:Lifted Jacobi}
        \frac{d^{2}J}{dt^{2}}+A\frac{dJ}{dt}+BJ+C=0,
    \end{align}
    which when expressed in coordinates, reads:
%    {\color{blue} I am considering using the summation notation verion of the lifted jacobi equation as it makes it easier to define A, B, C. See Below: - Josh}
    
    \begin{align}
        \label{eq:Lifted Jacobi - Summation Convention}
        \frac{d^{2}J^{c}}{dt^{2}}+A_{\ d}^{c}\frac{dJ^{d}}{dt}+B_{\ d}^{c}J^{d}+C^{c}=0\\ \nonumber
        A_{\ b}^{c}=2\Gamma_{\ db}^{c}\frac{dx^{b}}{dt}\\ \nonumber
        B_{\ d}^{c}=\Gamma_{\ db}^{c}\frac{d^{2}x^{b}}{dt^{2}}+\left(\Gamma_{\ ba,d}^{c}+\Gamma_{\ fd}^{c}\Gamma_{\ ab}^{f}\right)\frac{dx^{a}}{dt}\frac{dx^{b}}{dt}\\ \nonumber
        C^{c}=\frac{1}{2}g^{cd}\left(2g_{da;b}^{\prime}-g_{ab;d}^{\prime}\right)\frac{dx^{a}}{dt}\frac{dx^{b}}{dt}.
    \end{align}

    We note that $\Gamma_{\ fd}^{c}$ are the Christoffel symbols derived from the metric in equation \eqref{metric}, which are given by:

    \begin{align}
        \label{eq: Christoffel Bracket}
        \Gamma_{\ ab}^{d}=\frac{i}{2^{n+1}}\text{tr}\left(\mathcal{F}\left(d\right)\left(\left[a,\mathcal{G}\left(b\right)\right]+\left[b,\mathcal{G}\left(a\right)\right]\right)\right),
    \end{align}

    
        
    %We have defined several new things at this point, so we take a moment to clarify them all. The first of these, $\frac{dx^{b}}{dt}=H^{a}$ is the tangent vector to the Schr{\"o}dinger flow  curve $\gamma^a=U^a$, and $H\left(t;s\right)$ is a family of tangent vectors to the family of geodesics $U\left(t;s\right)$ relative to a family of metrics $g_{ab}\left(s\right)$, with 
    
    %\begin{align}
    %    g_{ab}^{\prime}=\left.\frac{\partial g_{ab}}{\partial s}\right|_{s=0}
    %\end{align}
